Join the Chat: How Curiosity Sparks Participation in Telegram Groups

This study delves into the mechanisms that spark user curiosity driving active engagement within public Telegram groups. By analyzing approximately 6 million messages from 29,196 users across 409 groups, we identify and quantify the key factors that stimulate users to actively participate (i.e., send messages) in group discussions. These factors include social influence, novelty, complexity, uncertainty, and conflict, all measured through metrics derived from message sequences and user participation over time. After clustering the messages, we apply explainability techniques to assign meaningful labels to the clusters. This approach uncovers macro categories representing distinct curiosity stimulation profiles, each characterized by a unique combination of various stimuli. Social influence from peers and influencers drives engagement for some users, while for others, rare media types or a diverse range of senders and media sparks curiosity. Analyzing patterns, we found that user curiosity stimuli are mostly stable, but, as the time between the initial message increases, curiosity occasionally shifts. A graph-based analysis of influence networks reveals that users motivated by direct social influence tend to occupy more peripheral positions, while those who are not stimulated by any specific factors are often more central, potentially acting as initiators and conversation catalysts. These findings contribute to understanding information dissemination and spread processes on social media networks, potentially contributing to more effective communication strategies.

==> text/backup/05_Conclusion_old.tex <==
\section{Conclusions and Future Work}
\label{sec:Conclusion}

% \ju{We should keep the same terms throughout the paper: curiosity stimulation profile, curiosity stimulation metrics, content sharing (or other term of preference), participation in group discussion (instead of engagement)? Choose one for each and keep it throughout the paper}

% This study explores user curiosity driving active engagement (i.e., content posting) in public Telegram groups and provides key insights into what stimulates user participation in group discussions. 
This study examines how the intrinsic human characteristic of curiosity drives active participation, specifically content posting, in public Telegram groups. It offers critical insights into the mechanisms that stimulate user engagement in group discussions. To the best of our knowledge, this is the first research to explore curiosity-driven engagement on the Telegram platform. 

Using 9 metrics that quantify different components of curiosity stimulation, we uncover  6 stimulus profiles.
% of curiosity stimuli driving users to participate in group discussions in Telegram. 
Two are mainly characterized by (direct/indirect) social influence. In contrast, three are dominated by other variables, notably novelty, uncertainty, or a mix of other stimuli. The last profile, in turn, has no clear evidence of being driven by any particular type of stimuli.  Interestingly, we found that direct and indirect social influence is a significant component of curiosity stimulation for 28\% of all messages, notably in groups categorized into the {\it Bookmaking, Cryptocurrencies, Linguistics, Darknet, and Software \& Application} topic.  
% \ju{Should we say this is counterintuitive given that Telegram is a social network? That is, once could expected a larger fraction. So it is interesting to highlight that there are other curiosity stimulation profiles also driving user behavior, even more often (again this contrasts to prior work that focused only on these two variables to infer profiles... Highlight the unexpected. }.
This result may sound counterintuitive because one could expect that social influence impacts more messages in Telegram since as a social network it should show significant social influence effects, as seen in both traditional social networks \cite{anagnostopoulos2008influence, aral2012identifying} and SMS/MMS networks \cite{peng2017social}. It is therefore noteworthy that other stimuli of curiosity are also influential in driving user participation (e.g., interest in using novel types of media account for roughly 7\% of the messages, while 32\% of the messages are driven by mixed stimuli), disputing previous studies that have only focused on social influence \cite{Sousa_Almeida_Figueiredo_2022b}. 
% % A large fraction of the messages are mainly elicited by other types of stimuli . 
% However, almost 22\% of the messages are not stirred by any of the identified stimuli (being referred to as curiosity independent).  
% Their curiosity stimulus thus remains unknown, opening the space for further investigation in the future. This highlights the complex social dynamics that shape users' interactions on the platform.
% \ju{Regarding the last sentence .I would not say their curiosity stimulus remains unknown. We do not know whether they are indeed driven by curiosity, by some component of stimulation that we did not capture in our metrics, or whether indeed curiosity is not a trigger. Not all message sharings must be driven by curiosity. So need to rephrase it somehow. }

Nevertheless, nearly 22\% of the messages are not influenced by any of the identified stimuli (referred to as curiosity independent). This suggests that these messages could be driven by other factors not captured by our metrics, such as the content of these messages, or they may not be driven by curiosity at all. This highlights the complex social dynamics influencing user engagement on the platform and indicates a need for further investigation.

%One of the main findings is that both direct and indirect social influence serve as significant components of curiosity stimulation for , with approximately 28\% of messages being influenced by one of these social factors.Others instead, are mainly elicited by other stimuli (e.g. impulse to utilize novel media is responsible for 6.8\% of messages). However, a noteworthy proportion of the messages are not stirred by any of the identified stimuli; their curiosity stimulus thus remains unknown, opening the space for further investigation in the future. This highlights the complex social dynamics that shape users' interactions on the platform.

% The stimuli that drive user participation tend to remain relatively stable during the period of analysis but may change over time. In particular, messages sent by the same user show some consistency in the type of stimuli that arouse their curiosity, focusing on specific areas of the curiosity stimulation space. However, as the time between messages increases, the likelihood of the user switching to a different stimulation profile increases. This suggests that although behaviour is generally stable, occasional variations in stimuli may trigger a change in how the user responds to group discussions. This implies that human curiosity is dynamic, responding to an interplay between changes in the external environment and the evolution of effective stimuli.  
% \ju{ "human curiosity is dynamic" seems to contradict what was said before (stable). I think this paragraph can be simplified and I suggest to explicitly mention "during the period of analysis".   I think you can say that: We observe that, during the period of analysis, despite some occasional changes in curiosity stimulation profile, the types of stimuli driving users to share content remain roughly stable. This allowed us to analyze profiles of curiosity stimulation at the user level for groups falling into different topics of discussion. We found that ....  }

We observe that as the time between messages increases, the likelihood of the user switching to a different stimulation profile increases. This confirms that human curiosity can be dynamic as already proven in \citet{sousa2019analyzing,Sousa_Almeida_Figueiredo_2022b}, responding to an interplay between changes in the external environment and the evolution of effective stimuli. 

Nevertheless, during the period of analysis, the curiosity stimulus profile which drives a user to share content remains roughly stable. This allowed us to analyze profiles of curiosity stimulation at the user level for groups falling into different topics of discussion. We see an emergence of a strong relationship between curiosity stimulus profiles and user engagement, highlighting how different stimuli shape participation patterns. Specifically, users engaged by uncertainty were more active, particularly in diverse and dynamic topics like \textit{Politics}, where the richness of discussion invites greater involvement. In contrast, those influenced by social factors, such as direct social influence, tended to post less frequently, often occupying more peripheral roles in the network. Notably, users who were not driven by any particular curiosity stimulus frequently emerged as conversation starters and central figures, underscoring the importance of understanding both individual curiosity profiles and the social dynamics at play. This insight sheds new light on how users contribute to and shape digital communities, with curiosity serving as a key driver of both active participation and leadership within group discussions.


% \ju{We are not discussing the radar graphs which are very interesting, they reveal different patterns of curiosity stimulation depending on topic. }

Eventually, the analysis of a dataset encompassing diverse discussion groups spanning various topics allows for insightful comparisons, revealing distinct patterns in curiosity stimulation that depend on the subject of the discussion. As previously mentioned, in certain topics, social influence heavily impacts many messages, while in others, such as \textit{Politics} and \textit{Technology}, uncertainty drives engagement. Additionally, there are topics like \textit{Video \& Films} and \textit{Software \& Applications} where the independent profile dominates, suggesting that in these groups, messages may not be primarily driven by curiosity.

% An interesting result is the emergence of a strong relationship between curiosity stimulus profiles and user engagement, highlighting how different motivations shape participation patterns. Specifically, users motivated by uncertainty were more active, particularly in diverse and dynamic topics like politics, where the richness of discussion invites greater involvement. In contrast, those influenced by social factors, such as direct social influence, tended to engage less frequently, often occupying more peripheral roles in the network. Notably, users who were not driven by any particular curiosity stimulus frequently emerged as conversation starters and central figures, underscoring the importance of understanding both individual curiosity profiles and the social dynamics at play. This insight sheds new light on how users contribute to and shape digital communities, with curiosity serving as a key driver of both active participation and leadership within group discussions.





% These findings offer valuable insights for improving online communities. By focusing on curiosity-driven engagement, content creators and platform developers can enhance participation through more stimulating and diverse content. Understanding what motivates users can also help in tackling challenges like misinformation by making it easier to identify and promote meaningful interactions. Ultimately, this research provides a practical framework for fostering healthier, more engaged digital communities where quality content and active participation thrive.

These findings provide valuable insights into the dynamics of online communities by exploring curiosity-driven engagement. 
By presenting this research, we enhance the understanding of how curiosity—an inherent human behavioral factor linked to cognition—drives both information dissemination and the spreading of information, an aspect that has been largely overlooked in prior work \cite{moreno2004dynamics,cornand2008optimal,wen2014sword,li2020characterizing}.

% \ju{Should we contrast these findings with the ones on WhatsApp? To the very least mention the fact that we uncover a larger fraction of messages that are not driven by social influence, whereas prior work focused only on profiles driven by social influence.}
% Future work includes 
Future works include examining how the content of messages triggers different types of curiosity and assessing how these triggers influence user engagement across various discussion platforms. This research will also explore how different types of curiosity stimulation impact long-term participation and community growth, aiming to understand the broader effects of these interactions on user involvement and community dynamics.

==> text/backup/05_Conclusion_old_old.tex <==
\section{Conclusion \todo{Work In Progress}}
\label{sec:Conclusion}
This study explores user engagement in public Telegram groups, providing key insights into what drives user participation. The analysis shows that social influence is a significant factor in engagement. Some users are heavily influenced by the activities of others in their groups, with both direct influence from immediate peers (24.9\%) and indirect influence from more influential users playing activist roles (7.8\%). Others instead, are mainly influenced by other stimuli (e.g. Novelty stimulus related to media usage for the 16.4\%). However, surprisingly, the relative majority of the users (31.2\%) is not affected by any of the identified stimuli; their curiosity stimulus thus remains unknown, opening the space for further future investigations. This highlights the complex social dynamics that shape user interactions on the platform.

The research further shows considerable variation in engagement patterns across different groups and topics. This suggests that the nature of the topic plays a significant role in how users interact. For example, seemingly unrelated topics like Cryptocurrencies and Software and Applications share a higher proportion of users stimulated by direct social influence. Conversely, in Technologies and Politics, the predominant stimulus comes from engaging in rich and varied conversations (high Uncertainty).

Lastly, the study finds that influence centrality, i.e. how central a user is to discussions, is influenced by these engagement drivers. Users motivated by direct social influence and user novelty are more pheriferical in the \textit{influence network}. This underscores the importance of these factors in stimulating and activating even users who are less likely to be influencers. In contrast, no evidence has emerged on the stimuli that lead the most central users to activate themselfs.

These findings have important implications for managing and designing online communities. For content creators and group administrators, focusing on producing novel, complex, and stimulating content can enhance user engagement. For platform developers, understanding these dynamics can inform the design of features that promote active and meaningful interactions.

In conclusion, understanding the drivers of user engagement helps in comprehending how information is disseminated and propagated within these groups. This is crucial for studying and addressing social threats such as misinformation. By identifying the factors that make certain messages more engaging, it becomes possible to understand how false information can spread rapidly and influence a large audience. Consequently, these insights can inform the development of strategies to mitigate the spread of misinformation and improve the overall quality of information shared within online communities.


==> text/backup/curiosity_metrics.tex <==
\subsection{Operational Definitions}
\label{subsec:Mathematical_Operationalization}






%Rewritten from this papers: https://www.sciencedirect.com/science/article/abs/pii/S2468696422000040

The curiosity driving the posting of a message by a given user $u$ at a given time $t$ depends on the past 
%has a period of activation $\Delta T$ , that is, a time interval preceding the user’s action (i.e., the posting of the message) during which
messages posted in the group (including messages posted by $u$ herself). % may contribute to stimulating $u$’s curiosity. 
Thus, a posting event at time t defines a window of interaction $[t ; t-\Delta T ]$. Messages posted before  $t-\Delta T$  are assumed to be too old to have any effect on $u$’s curiosity at time $t$.

We define the sets of users, groups, and types of media as $U,G,M$ respectively. We do not assume access to message content, as it may not be available. Instead, we use the different types of media used to compose the message content as a representation of it. %, that is, we define  $M$= \{‘‘text’’, ‘‘image’’, ‘‘audio’’, ‘‘video’’, ‘‘URL’’, ‘‘poll’’, ‘‘other’’\}. 
Each message under analysis is then a tuple $(u, C_m , g, t)$ indicating that it was posted by user $u\in U$ in group $g \in G$ at time $t$ with media types belonging to set $C_m \subseteq M$. Note that the same message may contain content in different media (e.g., a text and an image).
%We use notation $t_{i|u,g}$ to refer to the timestamp of the i-th message posted by user $u$ in group $g$. We assume time is continuous starting at 0. Thus, 
No two messages can be posted at exactly the same time in a group. Each group is composed of a set of users $U_g$. 

\paragraph{Novelty}

The metric $userNovelty$ captures the novelty related to the user $u$ posting the content. The idea is that the experience of posting content is less novel to users who already posted many messages in recent times, which ultimately affects the curiosity driving the action. User novelty measures how novel the posting experience is for the user with respect to the window of interaction. Given the  user $u$  posting a message at time $t$ in group $g$, the metric is computes as: 

$$userNov(u,t,g)=
\begin{cases}
    -\log_2 (\frac{n_{v|t,g}}{\sum_{v} n_{u|t,g}}) , & \text{if } n_{u|t,g}>0\\
    -\log_2 (1/|U_{t,g}|),              & \text{otherwise}
\end{cases}
$$

where $n_{v|t,g}$ is the number of messages sent in the window of interaction $[t ; t-\Delta T ]$ by any user $v$ (including $u$) in group $g$.  %$userNovelty$ varies between 0 and $+\infty$. 
If no previous message is sent by $u$, we set the novelty to its maximum value possible, which corresponds to the uniform distribution of users, i.e. $-\log_2 (1/|U_{t,g}|)$ where $U_{t,g}$ is the set of distinct users that posted content in group g during the current window of interaction. 

Similarly, we define a novelty metric related to the message categories, based on the surprisal (i.e., Shannon information content) associated with that variable:

% $$catNov(C_m,t,g)=
% \begin{cases}
%     -\log_2 (\frac{\sum_{c\in C_m}n_{c|t,g}}{|C_m|\sum_{k\in C}n_{k|t,g}}) , & \text{if } \sum_{c\in C_m}n_{c|t,g}>0\\
%     -\log_2 (1/|C_{t,g}|),              & \text{otherwise}
% \end{cases}
% $$


$$catNov(C_m,t,g)=
\begin{cases}
    -\log_2 (P_{t,g}(C_m)) , & \text{if } P_{t,g}(C_m)>0\\
    %\sum_{c\in C_m}n_{c|t,g}>0\\
    -\log_2 (1/|C_{t,g}|),              & \text{otherwise}
\end{cases}
$$

where $P_{t,g}(C_m)$ is the average probability of the media types posted in the message, which is estimated as $P_{t,g}(C_m)=\frac{1}{|C_m|} \sum_{c\in C_m}\frac{n_{c|t,g}}{\sum_{c'\in C_{t,g}}n_{c'|t,g}} $, 
with $C_{t,g}$ being the set of media types associated with all messages posted within the window of interaction. 
This metric captures how surprising it is that the message posted at time t contains the media types category in $C_m$. 

Both novelty metrics vary between 0 and $+\infty$.


\paragraph{Uncertainty}

Both novelty-related metrics focus on the user or the categories of the message posted in $t$. The aggregation of either metric for all messages (users or categories) posted in the window of interaction, using entropy, captures the uncertainty. 
The idea behind these metrics is that the curiosity of the user may be more/less stimulated by the greater/less variety in the users posting messages (and in the categories of these messages) during the window of interaction.
Thus, we define metrics of uncertainty related to users and categories as:

$$userUncert(t,g)= -\sum_{v\in U_{g}}  \frac{n_{v|t,g}}{\sum_{v'} n_{{v'}|t,g}} \log_2 (\frac{n_{v|t,g}}{\sum_{v'} n_{v'|t,g}})
$$

$$catUncert(t,g)= -\sum_{c\in C_{t,g}}  \frac{n_{c|t,g}}{\sum_{c'}n_{c'|t,g}}  \log_2 (\frac{n_{c|t,g}}{\sum_{c'}n_{c'|t,g}})
$$

Both uncertainty metrics vary between 0 and $1$.

%\lv{This is basically the homogeneity of users/type in the window of interaction}\gp{it is}

\paragraph{Conflict}

Conflict measures the diversity in the stimulus.
%might occur when the same stimulus triggers multiple different responses. 
The basic idea is that the distinct elements (categories/users) that appear in the window of interaction represent the different responses stimulating the curiosity of the user, and the strength of each response is captured by the probability of occurrence of each element (category/user).  
%We instantiate this variable by first computing the average probability of users (categories) over all users (message categories) in the window of interaction, and then taking the surprisal of the result. This procedure leads to two new metrics, one related to users and the other to categories: 
Thus, we define metrics of conflict related to users and categories to quantify the difference in terms of number of distinct users or distinct categories present in the window of interaction:


%$$userConflict(t,g)= - \log_2 (\frac{1}{|U_{t,g}|} \sum_{d\in U_{g}}  \frac{n_{d|t,g}}{\sum_u n_{u|t,g}})$$

% We instantiate this variable as the surprisal of the average probability of users (categories) over all users (message categories) in the window of interaction. This procedure leads to two new metrics, one related to users and the other to categories:

% $$userConflict(t,g)= - \log_2 (\frac{1}{|U_{t,g}|})
% $$

%\lv{Unsure: can userConflict be rewritten as  $- \log_2 (\frac{1}{|U_{t,g}|})$? }

$$userConflict(t,g)=  - \log_2 (\frac{1}{|U_{t,g}|})$$


%$$ catConflict(t,g)=  - \log_2 (\frac{1}{|C_{t,g}|} \sum_{c\in C_{t,g}} \frac{n_{c|t,g}}{\sum_{k\in C}n_{k|t,g}}) $$

$$ catConflict(t,g)=  - \log_2 (\frac{1}{|C_{t,g}|}) $$


Both conflicts vary between 0 and $+\infty$. Many users (categories) lead to large conflict. A single user (category) leads to no conflict, i.e., conflict 0.

%\lv{I don't see practical differences between conflict and uncertainty}
%\gp{conflict captures diversity (how many users (categories), while uncertainty captures homogeneity (did they all post the same number of messages?)}

\paragraph{Complexity}
An alternative form of capturing the diversity of message categories in the current window of interaction is by exploiting the unique occurrences of the media types. This metric, also based on surprisal, captures how many distinct categories of messages are posted during the current window of interaction. It is defined as:

$$
catComplex(t,g)=-\log_2(\frac{|C_{t,g}|}{|M|})
$$

$catComplex$ varies between 0 when all categories are present in the time window to $+\infty$ (when only a single category is present but there are infinity categories in general). 
%\lv{shouldn't be called simplicity instead of complexity since it is the opposite?} \gp{Agree, furthermore now I realised that $catComplex(t,g)= \log_2(\frac{1}{|C_{t,g}|})+\log_2(|M|))=-catConflict(t,g) +\log_2(|M|))$ but if it was true, the correlation between the metrics had to be always -1 (and it wasn't), then should be something wrong, or in the definitions, or in the code, or we missed something }

Note that complexity and conflict are functions of each other (and opposite). Indeed: $catComplex(t,g)= \log_2(\frac{1}{|C_{t,g}|})+\log_2(|M|))=-catConflict(t,g) +\log_2(|M|))$.

%Note that all the metrics defined are always non-negative and should be interpreted as: the greater the value the higher the stimulus to the curiosity of the destination user. \lv{debatable sentence}


\paragraph{Social curiosity}

To distinguish between the user whose curiosity we are analyzing, i.e., user $u$ who posted a message at time $t$ in group $g$ and the other users who may stimulate $u$’s curiosity through social influence, we refer to the former as the destination $d$ and the latter as origins $o$ of social influence. We define:

\begin{itemize}
    \item Probability of observing an origin $o$ on group $g$: 
    $P_{t,g}(O=o)$
    \item Probability of observing a destination $d$ on group $g$: 
    $P_{t,g}(D=d)$
    \item Probability of observing a destination $d$ given an origin $o$:
    $P_{t,g}(D=d|O=o)$
    \item Joint probability of observing a destination $d$ and an origin $o$: 
   $P_{t,g}(D=d,O=o)$
\end{itemize}

All these probabilities are conditioned on the group $g$ and timestamp $t$ of the current message and can be estimated given the message sequence history up to $t$.

We define two social curiosity metrics that are based on the concept of Pointwise Mutual Information ($PMI$), which is computed for a particular destination $d$ and origin $o$ as:

%or a pair of outcomes $x$ and $y$ belonging to discrete random variables $X$ and $Y$. The pointwise mutual information of a particular destination $d$ and a particular origin $o$ is defined as:

$$PMI_{t,g}(d,o)=
\begin{cases}
    \log_2 (\frac{P_{t,g}(d|o)}{P_{t,g}(d)}) , & \text{if } P_{t,g}(d)>0\\
    0,              & \text{otherwise}
\end{cases}
$$

%$PMI_{t,g}$ varies between $-\infty$ and $+\infty$. 
The $PMI$ of $d$ and $o$ measures the reduction in the uncertainty of destination $d$ posting a message due to the knowledge that $o$ also posted a message within the window of interaction.
It means that, based on historical patterns, the behavior of user $d$ in the group is influenced by the recent behavior of user $o$. Naturally, we set the $PMI$ value to 0 if there is no history of messages posted by $d$.
Note that $PMI$ is negative if $d$ and $o$ occur less frequently than would be expected under the assumption of independent behavior. Then, if there is no evidence of social influence of $o$ on $d$  (i.e. $PMI_{t,g}(d,o)\leq0$), we clip negative values of $PMI$ at 0, i.e., $PMI^+$.

Given that the current window of interaction may have multiple origins stimulating the curiosity of destination $d$, 
%we need to aggregate the mutual information computed for each origin $o$ that appears (except $d$). We do so by computing the average and 
we compute the maximum social influence for all origins $o$ on $d$.% We thus build two metrics capturing the average and the maximum direct influence of all the origins $o'$ in the window of interaction on the destination $d$, based on historical patterns.


%$$avgDirInf(d,t,g)=\frac{\sum_{o' \in O_{d,t,g}}PMI^+_{t,g}(d,o')}{|O_{d,t,g}|} $$

$$maxDirInf(d,t,g)=\max_{o \in O_{d,t,g}}PMI^+_{t,g}(d,o) $$

where $O_{d,t,g}$ is the set of origin for which we can reliably estimate $PMI$ at time t on group g for d.
%\lv{For me it makes sense the max, while the avg is too dependant on the amount of history. Notice that "reliably estimate" is a key factor: we might need a lots of message to estimate it.}\gp{We saw, as in \cite{Sousa_Almeida_Figueiredo_2022b}, that avg and max metrics are very correlated and in the end we both used max, but we can justify it in the paper with your argument} 

In addition to direct influence, we argue that some users may have a natural ability to influence others.
Users who often post content and, in doing so, keep the discussion going by driving others to also post content. We consider that, even in the absence of prior experiences such influencers may still stimulate the curiosity of a user (e.g., a newcomer) in the group. 

We identify these indirect influencers by searching for origins $o$ that tend to have a strong influence towards any destination $d'\in D$. Given this rationale, we propose a metric based on the mutual information of all the destinations conditioned on a particular origin, that is:

$$MI_{t,g}(D,o)=\sum_{d'\in U_g} P_{t,g}(d',o)PMI_{t,g}(d',o)$$

%$MI$ ranges between between $-\infty$ and $+\infty$.
Again, we clip non-positive values of mutual information at 0 (i.e., $MI^+$) as a reflection of no social influence from origin $o$ on any destination. Smaller values of $MI^+$ suggest weaker and no clear influence of $o$ over users. %The higher the value computed based on historical patterns, the higher the indirect influence that $o$ may have over a destination.

Again, we aggregate the above metric for all origins by taking the maximum one:
%for all origins $o' \in O_{d,t,g}$ in the window of interaction via the average and maximum functions, referring to them as average and maximum indirect influence:


%$$avgIndInf(d,t,g)=\frac{\sum_{o' \in O_{d,t,g}}MI^+_{t,g}(D,o')}{|O_{d,t,g}|} $$

$$maxIndInf(d,t,g)=\max_{o' \in O_{d,t,g}}MI^+_{t,g}(D,o') $$

The indirect social influence metrics are particularly useful to capture the influence that an origin $o$ may exhibit on a destination she has not interacted with yet, as a consequence of the influence she has on all the other users in the group. If this is a recurring pattern for a specific destination $d$, the direct influence metrics, computed based on $P_{t,g}(d|o)$, will rise as time passes.

Both social curiosity metrics vary between 0 and $+\infty$.
Note that in \cite{Sousa_Almeida_Figueiredo_2022b}, the authors also proposed to compute each metric based on the  {\it average} social influence. However, they found both maximum and average variants of each metric to be strongly correlated with each other, keeping only the maximum in their study.



